DODA: Adapting Object Detectors to Dynamic Agricultural Environments in Real-Time with Diffusion

Object detection has wide applications in agriculture, but domain shifts of diverse environments limit the broader use of the trained models. Existing domain adaptation methods usually require retraining the model for new domains, which is impractical for agricultural applications due to constantly changing environments. In this paper, we propose DODA ($D$iffusion for $O$bject-detection $D$omain Adaptation in $A$griculture), a diffusion-based framework that can adapt the detector to a new domain in just 2 minutes. DODA incorporates external domain embeddings and an improved layout-to-image approach, allowing it to generate high-quality detection data for new domains without additional training. We demonstrate DODA's effectiveness on the Global Wheat Head Detection dataset, where fine-tuning detectors on DODA-generated data yields significant improvements across multiple domains. DODA provides a simple yet powerful solution for agricultural domain adaptation, reducing the barriers for growers to use detection in personalised environments. The code is available at https://github.com/UTokyo-FieldPhenomics-Lab/DODA.

==> sec/4_experiment_copy.tex <==
\section{Experiment}
\label{sec:experiment}
By default, DODA employs latent diffusion (LDM) \cite{rombach2022high} as the base diffusion model. The pre-training of DODA is performed on the GWHD 2+ dataset, followed by post-training on the GWHD training set. The implementation details can be found in Appendix \ref{app:imple}. We use Fréchet Inception Distance (FID), Inception Score (IS), COCO Metrics, YOLO Score and Feature Similarity (FS) as evaluation metrics. Their specific definitions can be found in Appendix \ref{app:eval_metric}.

\subsection{Main Results}
\subsubsection{Synthetic Data for Agricultural Object Detection Domain Adaptation}
\label{subsec:DA}

We initialize a YOLOX-L \cite{ge2021yolox} model on the GWHD training set, serving as the baseline and base model.

Samples of data generated by DODA for different agricultural domains can be seen in the Fig.~\ref{fig:Overview} left. As shown in Table~\ref{t:domains_adaptation}, the data of 13 domains were collected from different devices, different regions and different stages of wheat head development. After fine-tuning the detector with domain-specific data synthesized by DODA, recognition across these domains improved, with an average improvement of 7.5. 

In addition to the GWHD, we test our method on wheat images collected by UAV, which have significantly different spatial resolutions. As shown in the Table~\ref{t:domains_adaptation}, our method can effectively help the detector adapt to UAV image data. Furthermore, we explore cross-crop adaption. As highlighted in the last row of Table~\ref{t:domains_adaptation}, our method successfully adapts the detector trained on wheat to sorghum \cite{ghosal2019weakly}. These results suggest our method effectively helps the detector adapt to new scenes of agricultural field, bridging the gap between limited manual annotations and complex, ever-changing agricultural environments. Appendix \ref{app:qualitative_da} illustrates the more generated data and example of adaption results.

\begin{table*}
  \caption{Domain-specific performance on GWHD test set after fine-tuning with DODA-generated data. Improvements over baseline are marked in \textcolor{red}{red} in parentheses. Consistent improvements across various domains demonstrate that DODA is effective in adapting detectors to new agricultural domains.
  }
  \label{t:domains_adaptation}
  \centering
  \setlength{\tabcolsep}{3.5pt}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
    \toprule
    Domain & AP & AP$_{50}$ & AP$_{75}$ & AP$^{s}$ & AP$^{m}$ & AP$^{l}$ & Development stage & Platform & Country\\
    \midrule
    \multicolumn{6}{l}{Global Wheat Head Detection} \\ 
    ARC\_1 & 35.0 & 29.7 & 8.1 & 35.0 & 39.9 & 73.1 & Filling & Handheld & Sudan \\
    \quad+ Ours & 37.4 (\textcolor{red}{+2.4}) & 78.3 (\textcolor{red}{+5.2}) & 32.3 (\textcolor{red}{+2.6}) & 8.3 (\textcolor{red}{+0.2}) & 36.8 (\textcolor{red}{+1.8}) & 43.0 (\textcolor{red}{+3.1}) &&&\\[1pt]
    CIMMYT\_1 & 26.7 & 65.7 & 16.9 & 5.3 & 24.6 & 45.9 & Postﬂowering & Cart & Mexico \\
    \quad+ Ours & 40.4 (\textcolor{red}{+13.7}) & 80.7 (\textcolor{red}{+15.0}) & 36.1 (\textcolor{red}{+19.2}) & 16.2 (\textcolor{red}{+10.9}) & 39.2 (\textcolor{red}{+14.6}) & 55.5 (\textcolor{red}{+9.6}) &&&\\[1pt]
    KSU\_1 & 37.1 & 72.0 & 34.9 & 9.5 & 40.1 & 51.5 & Postﬂowering & Tractor & US \\
    \quad+ Ours & 46.7 (\textcolor{red}{+9.6}) & 84.7 (\textcolor{red}{+12.7}) & 47.2 (\textcolor{red}{+12.3}) & 22.0 (\textcolor{red}{+12.5}) & 49.1 (\textcolor{red}{+9.0}) & 53.4 (\textcolor{red}{+1.9}) &&&\\[1pt]
    KSU\_2 & 34.9 & 74.0 & 29.6 & 6.9 & 38.3 & 58.7 & Postﬂowering & Tractor & US \\
    \quad+ Ours & 42.2 (\textcolor{red}{+7.3}) & 86.5 (\textcolor{red}{+12.5}) & 33.9 (\textcolor{red}{+4.3}) & 16.2 (\textcolor{red}{+9.3}) & 44.9 (\textcolor{red}{+6.6}) & 61.5 (\textcolor{red}{+2.8}) &&&\\[1pt]
    KSU\_3 & 27.4 & 67.8 & 16.2 & 6.0 & 26.5 & 42.6 & Filling & Tractor & US \\
    \quad+ Ours & 39.2 (\textcolor{red}{+11.8}) & 81.3 (\textcolor{red}{+13.5}) & 31.8 (\textcolor{red}{+15.6}) & 16.9 (\textcolor{red}{+10.9}) & 39.0 (\textcolor{red}{+12.5}) & 50.0 (\textcolor{red}{+7.4}) &&&\\[1pt]
    KSU\_4 & 22.7 & 56.3 & 14.6 & 1.2 & 22.6 & 40.6 & Ripening & Tractor & US \\
    \quad+ Ours & 38.3 (\textcolor{red}{+15.6}) & 75.1 (\textcolor{red}{+18.8}) & 34.1 (\textcolor{red}{+19.5}) & 10.0 (\textcolor{red}{+8.8}) & 39.3 (\textcolor{red}{+16.7}) & 49.4 (\textcolor{red}{+8.8}) &&&\\[1pt]
    Terraref\_1 & 11.3 & 33.1 & 5.1 & 1.0 & 13.1 & 43.6 & Ripening & Gantry & US \\
    \quad+ Ours & 20.7 (\textcolor{red}{+9.4}) & 54.6 (\textcolor{red}{+21.5}) & 10.6 (\textcolor{red}{+5.5}) & 4.1 (\textcolor{red}{+3.1}) & 24.0 (\textcolor{red}{+10.9}) & 43.2 (\textcolor{red}{-0.4}) &&&\\[1pt]
    Terraref\_2 & 9.1 & 23.7 & 5.2 & 0.6 & 12.3 & 31.7 & Filling & Gantry & US \\
    \quad+ Ours & 16.4 (\textcolor{red}{+7.3}) & 41.5 (\textcolor{red}{+17.8}) & 10.2 (\textcolor{red}{+5.0}) & 2.7 (\textcolor{red}{+2.1}) & 20.7 (\textcolor{red}{+8.4}) & 47.2 (\textcolor{red}{+15.5}) &&&\\[1pt]
    Ukyoto\_1 & 35.0 & 68.4 & 31.8 & 4.9 & 38.7 & 56.8 & Postﬂowering & Handheld & Japan \\
    \quad+ Ours & 35.6 (\textcolor{red}{+0.6}) & 70.1 (\textcolor{red}{+1.7}) & 32.6 (\textcolor{red}{+0.8}) & 5.5 (\textcolor{red}{+0.6}) & 39.0 (\textcolor{red}{+0.3}) & 57.3 (\textcolor{red}{+0.5}) &&&\\[1pt]
    UQ\_8 & 31.3 & 66.3 & 24.8 & 12.8 & 39.1 & 53.3 & Ripening & Handheld & Australia \\
    \quad+ Ours & 36.3 (\textcolor{red}{+5.0}) & 70.3 (\textcolor{red}{+4.0}) & 33.6 (\textcolor{red}{+8.8}) & 16.6 (\textcolor{red}{+3.8}) & 44.4 (\textcolor{red}{+5.3}) & 58.3 (\textcolor{red}{+5.0}) &&&\\[1pt]
    UQ\_9 & 30.9 & 66.8 & 25.6 & 8.4 & 35.0 & 54.4 & Filling-ripening & Handheld & Australia \\
    \quad+ Ours & 36.9 (\textcolor{red}{+6.0}) & 72.3 (\textcolor{red}{+5.5}) & 34.8 (\textcolor{red}{+9.2}) & 14.6 (\textcolor{red}{+6.2}) & 41.0 (\textcolor{red}{+6.0}) & 58.4 (\textcolor{red}{+4.0}) &&&\\[1pt]
    UQ\_10 & 37.7 & 78.5 & 31.2 & 20.7 & 43.7 & 53.8 & Filling-ripening & Handheld & Australia \\
    \quad+ Ours & 43.3 (\textcolor{red}{+5.6}) & 81.5 (\textcolor{red}{+3.0}) & 41.1 (\textcolor{red}{+9.9}) & 26.5 (\textcolor{red}{+5.8}) & 49.0 (\textcolor{red}{+5.3}) & 56.6 (\textcolor{red}{+2.8}) &&&\\[1pt]
    UQ\_11 & 27.8 & 69.5 & 16.4 & 17.0 & 34.0 & 42.0 & Postﬂowering & Handheld & Australia \\
    \quad+ Ours & 31.0 (\textcolor{red}{+3.2}) & 71.6 (\textcolor{red}{+2.1}) & 21.6 (\textcolor{red}{+5.2}) & 21.2 (\textcolor{red}{+4.2}) & 36.2 (\textcolor{red}{+2.2}) & 45.7 (\textcolor{red}{+3.7}) &&&\\[1pt]
    \midrule
    K & 13.3 & 35.5 & 6.6 & 9.0 & 18.0 & - & Ripening & UAV & - \\
    \quad+ Ours & 28.2 (\textcolor{red}{+14.9}) & 54.9 (\textcolor{red}{+19.4}) & 25.9 (\textcolor{red}{+19.3}) & 20.0 (\textcolor{red}{+11.0}) & 37.5 (\textcolor{red}{+19.5}) & - &&&\\[1pt]
    Sorghum & 17.3 & 40.0 & 12.6 & 17.7 & 21.5 & - & Ripening & UAV & Australia \\
    \quad+ Ours & 29.4 (\textcolor{red}{+12.1}) & 70.5 (\textcolor{red}{+30.5}) & 17.9 (\textcolor{red}{+5.3}) & 30.0 (\textcolor{red}{+12.3}) & 31.5 (\textcolor{red}{+10.0}) & - &&&\\[1pt]
    \bottomrule
  \end{tabular}
  }
\end{table*}

\subsubsection{Comparisons with Previous Domain Adaption Methods}
\label{subsec:compaer_DA}
In this section, we compare our method with existing domain adaptation approaches for adapting detectors to the \textbf{Terraref} domain. The \textbf{Terraref} a combination of \textbf{Terraref1} and \textbf{Terraref2}, which are the most challenging domains in the GWHD dataset. As shown in Table~\ref{t:compaer_DA}, our method achieves the best trade-off between accuracy and speed, requiring only 2 minutes for adaptation.

\begin{table}
  \caption{Adaptation results on the \textbf{Terraref} domain. The adaptation time is measured on a single consumer-grade GPU Nvidia 4090. Source free: source data is not required for adaptation.}
  \label{t:compaer_DA}
  \centering
  \resizebox{\linewidth}{!}{
  \setlength{\extrarowheight}{-1pt}
  \begin{tabular}{lccc}
    \toprule
    Method & Source free & AP\(_{50}\)\(\uparrow\) & Adaptation time\(\downarrow\) \\
    \midrule
    Faster-RCNN \\
    \multicolumn{1}{l|}{Soure Only} & - & 18.2 & - \\
    \multicolumn{1}{l|}{SWDA \cite{saito2019strong}} & \xmark & 7.0 & 4.5 hours \\
    \multicolumn{1}{l|}{AASFOD \cite{chu2023adversarial}} & \xmark & 13.7 & 21 hours\\
    \multicolumn{1}{l|}{HTCN \cite{chen2020harmonizing}} & \xmark &  21.7 & 2 hours \\
    \multicolumn{1}{l|}{IRG \cite{vs2023instance}} & \cmark &  22.1 & 1.2 hours \\
    \multicolumn{1}{l|}{MemCLR \cite{vs2023towards}} & \cmark &  22.7 & 3 min \\
    \multicolumn{1}{l|}{DODA (ours)} & \cmark &  \textbf{36.7} & \textbf{2 min} \\
    \midrule
    YOLOV5-X \\
    \multicolumn{1}{l|}{Soure Only} & - & 38.6 & - \\
    \multicolumn{1}{l|}{AsyFOD \cite{Gao_2023_CVPR}} & \xmark &  47.0 & 2.5 hours \\
    \multicolumn{1}{l|}{AcroFOD \cite{gao2022acrofod}} & \xmark &  50.5 & 2.5 hours \\
    \multicolumn{1}{l|}{DODA (ours)} & \cmark &  \textbf{53.6} & \textbf{2 min} \\
    \bottomrule
  \end{tabular}
  }
\end{table}

\subsubsection{Comparisons with Previous Layout-to-image Methods}
\label{subsec:L2I_coco}

\begin{table}
  \caption{L2I results on COCO-val2017. Our method achieves significant improvements in controllability compared to previous works. * indicates filtering of objects whose area ratio is less than 0.02 and images with more than 8 objects.}
  \label{t:coco-L2I}
  \centering
  
  \setlength{\tabcolsep}{3pt}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{6}{c}{YOLO Score\(\uparrow\)} & \multirow{2}{*}{FID\(\downarrow\)} & \multirow{2}{*}{IS\(\uparrow\)} \\
    \addlinespace[-0.8ex]
    \cmidrule(lr){2-7}
    & mAP & AP\(_{50}\) & AP\(_{75}\) & AP\(^{s}\) & AP\(^{m}\) & AP\(^{l}\) \\
    \addlinespace[-0.8ex]
    \midrule
    \(256 \times 256\) \\  
    \multicolumn{1}{l|}{PLGAN* \cite{wang2022interactive}} & 21.4 & 34.7 & 22.7 & 10.1 & 21.2 & 33.1 & 35.9  & 17.7\(\pm\)0.9 \\  
    \multicolumn{1}{l|}{LostGANv2* \cite{sun2021learning}} & 26.6 & 40.5 & 29.0 & 13.7 & 26.2 & 39.8 & 37.0  & 17.0\(\pm\)0.9 \\  
    \multicolumn{1}{l|}{LAMA* \cite{li2021image}} & 40.6 & 54.4 & 44.9 & 27.1 & 41.2 & 50.7 & 37.5  & 18.4\(\pm\)1.0 \\  
    \multicolumn{1}{l|}{LayoutDiffusion* \cite{zheng2023layoutdiffusion}} & 30.2 & 55.7 & 28.7 & 10 & 27.4 & 48.3 & \textbf{23.6} & 24.3\(\pm\)1.2 \\
    \multicolumn{1}{l|}{\textbf{LI2I (ours)}*} & \textbf{56.3} & \textbf{72.7} & \textbf{60.3} & \textbf{43.2} & \textbf{57.0} & \textbf{67.7} & 31.5 & \textbf{24.6\(\pm\)1.2} \\

    \cmidrule(lr){2-9}

    \multicolumn{1}{l|}{Real image} & 43.3 & 58.9 & 46.6 & 29.7 & 61.8 & 74.7 & - & 29.0\(\pm\)1.3 \\
    \multicolumn{1}{l|}{LayoutDiffusion \cite{zheng2023layoutdiffusion}} & 6.3 & 15.2 & 4.2 & 0.6 & 8.4 & 24.7 & \textbf{20.5}  & 21.8\(\pm\)1.1 \\
    \multicolumn{1}{l|}{GeoDiffusion \cite{chen2023integrating}} & 29.2 & 40.5 & 30.9 & 9.2 & 52.4 & \textbf{72.2} & 34.3  & 24.7\(\pm\)1.1 \\
    \multicolumn{1}{l|}{ControlNet M2I \cite{zhang2023adding}} & 31.6 & 41 & 33 & 17.8 & 48 & 58.9 & 49.1  & 18.4\(\pm\)0.9 \\
    \multicolumn{1}{l|}{\textbf{LI2I (ours)}} & \textbf{34.3} & \textbf{47.8}  & \textbf{35.6}  & \textbf{19.9}  & \textbf{51.3}  & 67.8 & 29.9  & \textbf{28.5\(\pm\)0.8} \\
    \midrule
    \(512 \times 512\) \\
    \multicolumn{1}{l|}{GLIGEN*} & 42.1 & - & - & - & - & - & 30.7  & 26.8 \\
    \multicolumn{1}{l|}{MIGC*} & 39.1 & - & - & - & - & - & 31.4  & 26.1 \\
    \multicolumn{1}{l|}{CreatiLayout*} & 47.8 & - & - & - & - & - & 29.3  & 30.26 \\

    \cmidrule(lr){2-9}

    \multicolumn{1}{l|}{Real image} & 52.9 & 70.1 & 57.5 & 33.8 & 58.5 & 70.9 & - & 31.5\(\pm\)1.2 \\
    \multicolumn{1}{l|}{GeoDiffusion \cite{chen2023integrating}} & 29.4 & 42.3 & 31.3 & 1.1 & 26.8 & \textbf{64.3} & 28.8  & 26.4\(\pm\)2.4 \\
    \multicolumn{1}{l|}{ControlNet M2I \cite{zhang2023adding}} & 43.3 & 53.2 & 45.6 & 20.8 & 47.5 & 64.0 & 33.9  & 21.3\(\pm\)0.8 \\
    \multicolumn{1}{l|}{\textbf{LI2I (ours)}} & \textbf{45.2}  & \textbf{58.8}  & \textbf{48.0}  & \textbf{25.2}  & \textbf{50.7}  & \textbf{64.0}  & \textbf{24.9}  & 29.4\(\pm\)1.1 \\
    \bottomrule
  \end{tabular}
  }
\end{table}



Consistent with previous L2I studies, we perform experiments on the COCO dataset to demonstrate the effectiveness of our proposed method. Table~\ref{t:coco-L2I} shows that our LI2I method significantly outperforms all previous L2I methods in terms of controllability (mAP), while maintaining high image quality (FID) and diversity (IS). Moreover, in contrast to previous methods that represent layouts as text (LayoutDiffusion, Layout diffuse, GeoDiffusion), our layout images technique overcomes limitations of text-based layouts, allowing for more precise and detailed control, including small objects that were previously challenging to produce (AP$^s$). ControlNet \cite{zhang2023adding} takes semantic masks as conditions, and can achieve relatively accurate layout control, but it imposes stricter constraints, leading to much lower image quality and diversity. More importantly, using algorithms to obtain masks is challenging, making M2I unsuitable for data generation. The quantitative comparison of above methods can be found in Appendix \ref{app:qualitative_comparisons_coco}.

Furthermore, the YOLO Score achieved on our generated images closely approximate those obtained from real images. This close alignment highlights the accuracy of our synthetic labels, and indicates significant progress in narrowing the gap between synthetic and real data. 

Among methods (Layout diffuse, GeoDiffusion) based on LDM \cite{rombach2022high}, our method achieves the lowest FID. However, the FID is still relatively high compared to LayoutDiffusion, which does not use the variational autoencoder \cite{kingma2013auto}. To enhance the quality of the generated data, image quality needs further improvement.

\subsection{Ablation study}
\label{subsec:AB}

In this section, we perform ablation studies to evaluate the impact of each design and setting of the proposed method, additional results are in Appendix \ref{app:more_AB}. 

\noindent \textbf{Scaling dataset and GWHD 2+.} The separation of domain features by the domain encoder enables us to pre-train the diffusion model using a larger set of images, without requiring labels. In Table~\ref{t:pre-training-size}, we explore the effect of the proposed two-stage training. We consider two scenarios: target domain images are accessible (\textbf{w/ target images}) or inaccessible (\textbf{w/o target images}) during pre-traing.

As shown in Table~\ref{t:pre-training-size}, when no additional unlabeled data is used, training is one-stage, leading to the worst results. As the size of the pre-training dataset increases, the AP$_{50}$ steadily improves, demonstrating the effectiveness of the two-stage training process. Notably, pre-training diffusion models with unlabeled images from the target domain significantly enhances data quality. To support pre-training, we collect GWHD 2+, an extension of GWHD with 65k additional unlabeled wheat images from 12 domains. As shown in last row of Table~\ref{t:pre-training-size}, GWHD 2+ further improves the data quality and narrows the gap between w/ and w/o access to target images. The performance gains from pre-training with additional unlabeled images, particularly those from the target domain, suggest that our GWHD 2+ dataset is still insufficiently large. A priority for the future is to collect more images to enhance DODA's ability.

\noindent \textbf{Domain encoder.} Table~\ref{t:vision-encoders} shows the effect of the Domain encode. Without domain encoder, diffusion randomly samples from the training set, leading to lower FS. Independently of the architecture and training data, various pre-trained vision models can guide diffusion to generate image with specific features. Using ViT as the backbone, CLIP performs the best, while MAE \cite{he2022masked} worse than ResNet \cite{he2016deep}. Compared to contrastive learning, MAE focuses more on high-frequency texture features \cite{park2023self, vanyan2023analyzing}, which we hypothesize affects the quality of the domain embedding. To explore this, we test features from different MAE layers, as shallow layers are generally associated with high-frequency, low-level features. As shown in Table~\ref{t:mae-layers}, using shallower MAE features further impacts image quality.

\noindent \textbf{Position to merge the layout embedding.} Table~\ref{t:layout-merge-layers} presents the impact of layout embedding fusion position on layout controllability. It can be seen that fusing layout embedding with the layers of denoising U-Net decoder can more effectively convey layout information.

\begin{table}
  \caption{Impact of pre-training dataset size on the quality of generated data, measured by AP$_{50}$. Pre-training diffusion models with more unlabeled images, especially those from the target domain, can improve data quality.}
  \label{t:pre-training-size}
  \centering
  \begin{tabular}{lcccccc}
    \toprule
    Dataset Size & w/o target images & w/ target images \\
    \midrule
    33k & 41.1 & 41.1 \\
    45k & 44.8 & 45.4 \\
    56k & 45.4 & 49.6 \\
    121k & 48.4 & 50.7\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[!t]
  \centering
  \begin{minipage}{0.5\linewidth}
  \caption{Ablations on domain encoder.}
  \makeatletter\def\@captype{table}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lc}
      \toprule
      Domain Encoder & FS$\uparrow$\\
      \midrule
      \xmark & 0.477 \\
      CLIP & \textbf{0.769} \\
      MAE & 0.747 \\
      ResNet101 & 0.751 \\
      \bottomrule
    \end{tabular}
    }
  \label{t:vision-encoders}
  \end{minipage}
  \hfill
  \begin{minipage}{0.43\linewidth}
    \caption{Features from different layers in MAE as domain embedding.}
    \makeatletter\def\@captype{table}
    \renewcommand\arraystretch{0.9}
    \resizebox{\textwidth}{!}{
      \begin{tabular}{lcc}
        \toprule
        Layers & FS$\uparrow$ & FID$\downarrow$ \\
        \midrule
        2 & 0.622 & 44.8 \\
        4 & 0.664 & 37.7 \\
        8 & 0.719 & 30.6 \\
        12 & 0.747 & 28.0 \\
        \bottomrule
      \end{tabular}
      }
    \label{t:mae-layers}
    \end{minipage}
\end{table}


\begin{table}
  \caption{Ablations on the position to merge the layout embedding.}
  \label{t:layout-merge-layers}
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccc}
      \toprule
      \multirow{2}{*}{Encoder} & \multirow{2}{*}{Decoder} & \multicolumn{6}{c}{YOLO Score\(\uparrow\)} & \multirow{2}{*}{FID\(\downarrow\)}  \\
      \cmidrule(lr){3-8}
      && mAP & AP\(_{50}\) & AP\(_{75}\) & AP\(^{s}\) & AP\(^{m}\) & AP\(^{l}\) \\
      \cmidrule(r){1-2}
      \cmidrule(r){3-9}
      \xmark & \cmark & 23.1 & 64.1 & 10.2 & 17.1 & 28.2 & 22.0 & 27.2\\
      \cmark & \xmark & 26.0 & 69.5 & 12.5 & 20.5 & 30.7 & 21.8 & 27.7\\
      \cmark & \cmark & 25.3 & 67.5 & 11.9 & 18.8 & 30.7 & 23.1 & 27.3\\
      \bottomrule
    \end{tabular}
  }
\end{table}
